EfficientVITON: An Efficient Virtual Try-On Model using Optimized Diffusion Process

Would not it be much more convenient for everybody to try on clothes by only looking into a mirror ? The answer to that problem is virtual try-on, enabling users to digitally experiment with outfits. The core challenge lies in realistic image-to-image translation, where clothing must fit diverse human forms, poses, and figures. Early methods, which used 2D transformations, offered speed, but image quality was often disappointing and lacked the nuance of deep learning. Though GAN-based techniques enhanced realism, their dependence on paired data proved limiting. More adaptable methods offered great visuals but demanded significant computing power and time. Recent advances in diffusion models have shown promise for high-fidelity translation, yet the current crop of virtual try-on tools still struggle with detail loss and warping issues. To tackle these challenges, this paper proposes EfficientVITON, a new virtual try-on system leveraging the impressive pre-trained Stable Diffusion model for better images and deployment feasibility. The system includes a spatial encoder to maintain clothings finer details and zero cross-attention blocks to capture the subtleties of how clothes fit a human body. Input images are carefully prepared, and the diffusion process has been tweaked to significantly cut generation time without image quality loss. The training process involves two distinct stages of fine-tuning, carefully incorporating a balance of loss functions to ensure both accurate try-on results and high-quality visuals. Rigorous testing on the VITON-HD dataset, supplemented with real-world examples, has demonstrated that EfficientVITON achieves state-of-the-art results.

==> Sections/Related_Work/Evolution_of_Generative_Models_in_Virtual_Try-On.tex <==
Virtual try-on systems have become a cornerstone of contemporary e-commerce, allowing users to see how clothing items would look on them without the need for physical trials. Early approaches relied on 2D image warping and stitching techniques, which often fell short when handling complex poses, textures, or lighting variations. The emergence of deep learning, particularly generative models, has transformed this field by enabling more realistic and scalable solutions. In recent years, advances in diffusion models have further pushed the limits of image synthesis, delivering exceptional quality and stability in virtual try-on applications \cite{tryondiffusion}\cite{stableviton}.

Also, the evolution of Generative Models in Virtual Try-On Generative models, particularly Generative Adversarial Networks (GANs), have become a cornerstone of virtual try-on systems due to their ability to generate highly realistic images. Despite their popularity, GANs face several challenges, including mode collapse, training instability, and difficulties in preserving fine details in high-resolution outputs. As an alternative, diffusion models have gained traction by employing iterative denoising processes to produce high-quality images with greater stability. Recent advancements have showcased the potential of diffusion models in addressing fashion-specific challenges, including their application in virtual try-on tasks \cite{DCIVITON}\cite{ladivton}.

Over the past five years, virtual try-on systems have advanced significantly as researchers explore new models and techniques to overcome critical challenges, such as pose alignment, texture preservation, and image realism. Below is an overview of the key approaches, their contributions, and their limitations:
    \begin{enumerate}
        \item \textbf{Geometric Warping-Based Models}
        \par Early virtual try-on systems heavily relied on geometric warping techniques to align clothing items with the target body pose.
        These methods typically employed 2D image transformations, such as Thin Plate Spline (TPS), to warp garments onto the user’s image. For instance, VITON \cite{han2018viton} introduced a TPS-based warping approach that enhanced alignment but struggled to preserve fine details and textures. While computationally efficient, these methods often produced unrealistic results when dealing with complex poses, occlusions, or fabric deformations.\\
        \textbf{Strengths:} Low computational cost and straightforward implementation. \\
        \textbf{Weaknesses:} Poor handling of complex poses, textures, and overall realism.
        \item \textbf{GAN-Based Models}
In addition, the advent of GANs revolutionized virtual try-on systems by enabling the realistic synthesis of garments on target poses. These methods generally operate in two stages: first, a warping module aligns the clothing with the body, followed by a refinement module that generates the final output. For example, VITON \cite{han2018viton} and CP-VTON \cite{wang2018characteristic} are GAN-based frameworks that combined pose estimation with texture preservation to achieve state-of-the-art results. However, GANs often face issues such as training instability, visible artifacts, and challenges in preserving fine details.
        
        \textbf{Strengths:} High-quality realism and the ability to handle intricate textures. \\
        \textbf{Weaknesses:} Unstable training, artifact generation, and difficulty preserving details.
        \item \textbf{Attention-Based Models}
        \par To address GANs’ limitations, attention mechanisms were introduced to enhance alignment and texture preservation. These models use attention maps to focus on relevant regions of the clothing and the body, enabling more precise alignment and detailed output. For example, CP-VTON+ \cite{issenhuth2020parserfree} developed an attention-based try-on network that excelled at managing complex patterns and textures. However, attention-based models tend to be computationally intensive and require large datasets for training.
        
        \textbf{Strengths:} Better alignment and improved texture detail. \\
        \textbf{Weaknesses:} High computational cost and heavy data requirements.
        
        \item \textbf{Diffusion Models}
Recently, diffusion models have emerged as a powerful alternative to GANs in virtual try-on applications. Unlike GANs, these models iteratively denoise images, which enhances stability and output quality. They have proven highly effective at managing complex textur \cite{tryondiffusion} and Stable-VITON \cite{stableviton} are diffusion-based models that demonstrate exceptional image quality and stability. However, their iterative nature makes them computationally expensive, which poses challenges for real-time applications.
        
        \textbf{Strengths:} Exceptional image quality, stability, and detail preservation. \\
        \textbf{Weaknesses:} High computational demands and slow inference speeds.

        \item \textbf{Hybrid Models}
        \par Hybrid models combine the strengths of multiple approaches, such as geometric warping, GANs, and attention mechanisms, to achieve better alignment, realism, and efficiency. For instance, HR-VITON \cite{hrVITON} proposed a hybrid framework that integrates geometric warping for initial alignment with GAN-based refinement for final synthesis. While effective, hybrid models often require complex architectures and significant tuning.
        
        \textbf{Strengths:} Balanced performance by leveraging multiple techniques. \\
        \textbf{Weaknesses:} Complex architecture and intensive tuning requirements.
    
        \item \textbf{Multi-Modal Models}
        \par Advancements in multi-modal inputs, such as text descriptions and sketches, have enhanced user interaction and personalization in virtual try-on systems. For example, Text2Cloth \cite{ren2021clothtransformer} developed a system allowing users to describe clothing in natural language, which the model then synthesizes onto their image. Similarly, Sketch2TryOn \cite{xie2021patchgan} introduced a sketch-based interface for designing and visualizing custom clothing in real-time. While engaging, these methods require additional preprocessing and are computationally expensive.
        
        \textbf{Strengths:} Greater personalization and user engagement. \\
        \textbf{Weaknesses:} High computational cost and preprocessing demands.
    
    \end{enumerate}
    
Diffusion-based methods currently lead the field, generating high-resolution, photorealistic images that preserve intricate clothing details. Recent advancements include integrating pose estimation, attention mechanisms for alignment, and multi-modal inputs for personalization. However, challenges such as adapting to diverse body shapes, managing occlusions, and improving real-time performance remain unresolved.

Despite significant progress, several gaps persist in virtual try-on research. Current methods often focus solely on static images, underutilizing temporal data for video-based try-on systems \cite{densepose}. Personalization, such as accommodating user preferences or diverse body types, remains limited. The computational cost of diffusion models also restricts their use in real-time applications. Furthermore, there is a lack of standardized evaluation metrics tailored to virtual try-on systems, complicating objective comparisons between methods \cite{issenhuth2020parserfree}.

While existing systems have improved realism and usability, many struggle to generalize across diverse datasets and real-world scenarios. For instance, GAN-based methods often generate artifacts in complex scenarios, while diffusion models, despite their stability, remain computationally expensive \cite{tryondiffusion}\cite{stableviton}. Additionally, most systems rely on paired datasets, limiting scalability.

The research proposes a diffusion model framework to improve virtual try-on experiences, utilizing non-uniform time steps, temporal coherence, and personalization to reduce computational demands and enhance image quality.



==> Sections/Results/Efficiency_Results.tex <==
This section presents the qualitative, quantitative, and efficiency evaluation of EfficientVITON, demonstrating its superior performance in virtual try-on.

\subsection{Qualitative Results}

EfficientVITON generates visually realistic and accurate virtual try-on images (Fig. \ref{fig:qualitative_results}), effectively handling complex clothing patterns, text, logos, and varying body types and poses.  The model preserves intricate clothing details, maintains natural folds and shadows, and adapts seamlessly to different garment coverage levels, producing results visually indistinguishable from real photographs.

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.850\textwidth]{Sections/Results/images/MixCollage-18-Jan-2025-12-57-PM-9897.jpg}
  \caption{Qualitative Results on VITON-HD.}
  \label{fig:qualitative_results}
\end{figure*}


\subsection{Quantitative Results}

Quantitative evaluation using FID \cite{FID} and LPIPS \cite{LPIPS} (Table \ref{tab:comparison}) demonstrates EfficientVITON's superior performance.  The model achieves a lower FID score than state-of-the-art methods, indicating higher realism. While LPIPS scores are competitive, the RePaint \cite{RePaint} refinement further improves performance in paired settings by addressing potential reconstruction errors related to the agnostic map.  EfficientVITON's consistent performance across different experimental setups highlights its robustness and generalizability.

\setlength{\tabcolsep}{20pt}
\begin{table}[h!]
\centering
\begin{tabular}{lll} \toprule
Method & LPIPS  & FID \\ \midrule
VITON-HD \cite{vitonhd} & 0.117  & 12.117 \\
HR-VITON \cite{hrVITON} & 0.1045  & 11.265\\ 
LADI-VTON \cite{ladivton} & 0.0964 & 9.480 \\
Paint-by-Example  \cite{PaintbyExample} & 0.1428 & 11.939 \\
DCI-VTON \cite{DCIVITON} & 0.0804  & 8.754 \\
GP-VTON \cite{GP-VTON} & 0.088 & 9.072 \\\midrule
Ours & 0.0842 & 8.703  \\
Ours (RePaint) & 0.0762 & 8.433 \\\bottomrule
\end{tabular}
\caption{Quantitative Comparison (Lower is Better).}
\label{tab:comparison}
\end{table}


\subsection{Efficiency Results}

The non-uniform timestep sampling strategy significantly improves efficiency (Table \ref{tab:efficiency}), reducing both training and inference times. The inference time is reduced by 72.4\%, enabling near real-time performance, while training time is reduced by 45.3\%, facilitating faster model development and experimentation.  These improvements enhance practicality for real-world applications and resource-constrained environments.

\setlength{\tabcolsep}{20pt}
\begin{table}[h!]
\centering
\begin{tabular}{lll} \toprule
Method & Training time & Inference Time \\ \midrule
Before & 1570 h & 58 s \\
After & 859 h & 16 s \\ \bottomrule
\end{tabular}
\caption{Comparison of Training time and Inference time for our model before and After using our new approach of applying the non-uniform timestep distribution.}
\label{tab:efficiency}
\end{table}

